Persistent Homology of Configuration Spaces of Trees

Multiparameter persistence modules come up naturally in topological data analysis and topological robotics. Given a metric graph $(X,\delta)$, the second configuration space of $(X,\delta)$ with proximity parameters (for example, the minimum distance allowed between each pair of robots) can be interpreted as a collection of all possible configurations of two robots moving in $(X,\delta)$. In this project, we study the $2$-parameter persistence modules associated with the second configuration spaces of the star graph ($\mathsf{Star}_k$, $k\geq 3$) and the generalized H-graph ($\mathcal{H}_{m,n}$, $m,n\geq 3$) with the edge length parameter $L_e$ and the restraint parameter $r$. Moreover, we provide the indecomposable direct summands for each persistence module.

==> app.tex <==
%% This BibTeX bibliography file was created using BibDesk.
%% https://bibdesk.sourceforge.io/

%% Created for WENWEN LI at 2023-03-09 22:18:10 -0600 


%% Saved with string encoding Unicode (UTF-8) 



@article{dover2013homeomorphism,
	Author = {Dover, James and {\"O}zaydin, Murad},
	Journal = {IMRN: International Mathematics Research Notices},
	Number = {20},
	Title = {Homeomorphism types of restricted configuration spaces of metric graphs.},
	Volume = {2018},
	Year = {2018}}

@article{abrams2002finding,
	Author = {Abrams, Aaron and Ghrist, Robert},
	Journal = {The American mathematical monthly},
	Number = {2},
	Pages = {140--150},
	Publisher = {Taylor \& Francis},
	Title = {Finding topology in a factory: configuration spaces},
	Volume = {109},
	Year = {2002}}

@article{ghrist2008barcodes,
  title={Barcodes: the persistent topology of data},
  author={Ghrist, Robert},
  journal={Bulletin of the American Mathematical Society},
  volume={45},
  number={1},
  pages={61--75},
  year={2008}
}

@article{BL15,
	Author = {Bauer, Ulrich and Lesnick, Michael},
	Journal = {arXiv preprint arXiv:1311.3681},
	Title = {Induced matchings and the algebraic stability of persistence barcodes},
	Year = {2013}}

@article{Botman-2015,
	Author = {Botnan, Magnus},
	Journal = {Proceedings of the American Mathematical Society},
	Number = {8},
	Pages = {3571--3577},
	Title = {Interval decomposition of infinite zigzag persistence modules},
	Volume = {145},
	Year = {2017}}



@article{B2014,
	Author = {Bubenik, Peter and Scott, Jonathan A},
	Journal = {Discrete \& Computational Geometry},
	Number = {3},
	Pages = {600--627},
	Publisher = {Springer},
	Title = {Categorification of persistent homology},
	Volume = {51},
	Year = {2014}}

@article{BE-2020,
	Author = {Buchet, Micka{\"e}l and Escolar, Emerson G},
	Journal = {arXiv preprint arXiv:2012.02467},
	Title = {The whole in the parts: Putting $n$D persistence modules inside indecomposable $(n+1)$D ones},
	Year = {2020}}

@article{BE-2019,
	Author = {Buchet, Micka{\"e}l and Escolar, Emerson G},
	Journal = {Journal of Applied and Computational Topology},
	Number = {3},
	Pages = {387--424},
	Publisher = {Springer},
	Title = {Every $1$D persistence module is a restriction of some indecomposable $2$D persistence module},
	Volume = {4},
	Year = {2020}}

%@article{C2009,
	%Author = {Carlsson, Gunnar},
	%Journal = {Bulletin of the American Mathematical Society},
	%Number = {2},
	%Pages = {255--308},
	%Title = {Topology and data},
	%Volume = {46},
	%Year = {2009}}

%@article{carlsson2005persistence,
	%Author = {Carlsson, Gunnar and Zomorodian, Afra and Collins, Anne and Guibas, Leonidas J},
	%Journal = {International Journal of Shape Modeling},
	%Number = {02},
	%Pages = {149--187},
	%Publisher = {World Scientific},
	%Title = {Persistence barcodes for shapes},
	%Volume = {11},
	%Year = {2005}}

@article{CZ2009,
	Author = {Carlsson, Gunnar and Zomorodian, Afra},
	Journal = {Discrete \& Computational Geometry},
	Number = {1},
	Pages = {71--93},
	Publisher = {Springer},
	Title = {The theory of multidimensional persistence},
	Volume = {42},
	Year = {2009}}

@article{zomorodian2005computing,
	Author = {Zomorodian, Afra and Carlsson, Gunnar},
	Journal = {Discrete \& Computational Geometry},
	Number = {2},
	Pages = {249--274},
	Publisher = {Springer},
	Title = {Computing persistent homology},
	Volume = {33},
	Year = {2005}}

@article{2021,
	Author = {Carlsson, Gunnar and Dwaraknath, Anjan and Nelson, Bradley J},
	Journal = {arXiv preprint arXiv:1911.10693},
	Title = {Persistent and zigzag homology: A matrix factorization viewpoint},
	Year = {2019}}

@article{CV-2008,
	Author = {Carlsson, Gunnar and De Silva, Vin},
	Journal = {Foundations of computational mathematics},
	Number = {4},
	Pages = {367--405},
	Publisher = {Springer},
	Title = {Zigzag persistence},
	Volume = {10},
	Year = {2010}}

@inproceedings{CVD,
	Author = {Carlsson, Gunnar and De Silva, Vin and Morozov, Dmitriy},
	Booktitle = {Proceedings of the twenty-fifth annual symposium on Computational geometry},
	Pages = {247--256},
	Title = {Zigzag persistent homology and real-valued functions},
	Year = {2009}}

@article{CV-2011,
	Author = {Tausz, Andrew and Carlsson, Gunnar},
	Journal = {arXiv preprint arXiv:1108.3545},
	Title = {Applications of zigzag persistence to topological data analysis},
	Year = {2011}}

@article{crawley2015decomposition,
	Author = {Crawley-Boevey, William},
	Journal = {Journal of Algebra and its Applications},
	Number = {05},
	Pages = {1550066},
	Publisher = {World Scientific},
	Title = {Decomposition of pointwise finite-dimensional persistence modules},
	Volume = {14},
	Year = {2015}}

@article{botnan2020decomposition,
  title={Decomposition of persistence modules},
  author={Botnan, Magnus and Crawley-Boevey, William},
  journal={Proceedings of the American Mathematical Society},
  volume={148},
  number={11},
  pages={4581--4596},
  year={2020}
}



@article{CSEH2007,
	Author = {Cohen-Steiner, David and Edelsbrunner, Herbert and Harer, John},
	Journal = {Discrete \& computational geometry},
	Number = {1},
	Pages = {103--120},
	Publisher = {Springer},
	Title = {Stability of persistence diagrams},
	Volume = {37},
	Year = {2007}}

@phdthesis{Dee,
	Author = {Deeley, Kenneth},
	School = {Durham University},
	Title = {Configuration spaces of thick particles on graphs},
	Year = {2011}}

@article{MM17,
	Author = {Meehan, Killian and Meyer, David},
	Journal = {arXiv preprint arXiv:1710.02858},
	Title = {An isometry theorem for generalized persistence modules},
	Year = {2017}}

@article{L15,
	Author = {Lesnick, Michael},
	Journal = {Foundations of Computational Mathematics},
	Number = {3},
	Pages = {613--650},
	Publisher = {Springer},
	Title = {The theory of the interleaving distance on multidimensional persistence modules},
	Volume = {15},
	Year = {2015}}

@article{MK2018,
	Author = {Kim, Woojin and M{\'e}moli, Facundo},
	Journal = {Journal of Applied and Computational Topology},
	Number = {4},
	Pages = {533--581},
	Publisher = {Springer},
	Title = {Generalized persistence diagrams for persistence modules over posets},
	Volume = {5},
	Year = {2021}}

@article{otter2017roadmap,
	Author = {Otter, Nina and Porter, Mason A and Tillmann, Ulrike and Grindrod, Peter and Harrington, Heather A},
	Journal = {EPJ Data Science},
	Pages = {1--38},
	Publisher = {Springer},
	Title = {A roadmap for the computation of persistent homology},
	Volume = {6},
	Year = {2017}}

@article{chazal2017introduction,
	Author = {Chazal, Fr{\'e}d{\'e}ric and Michel, Bertrand},
	Journal = {arXiv preprint arXiv:1710.04019},
	Title = {An introduction to topological data analysis: fundamental and practical aspects for data scientists},
	Year = {2017}}

@book{2007,
	Author = {Hazewinkel, Michiel and Gubareni, Nadiya and Kirichenko, Vladimir V},
	Publisher = {Springer Science \& Business Media},
	Title = {Algebras, rings and modules},
	Volume = {1},
	Year = {2004}}

@book{erdmann2018algebras,
	Author = {Erdmann, Karin and Holm, Thorsten},
	Publisher = {Springer},
	Title = {Algebras and representation theory},
	Year = {2018}}

@article{carlsson2009topology,
	Author = {Carlsson, Gunnar},
	Journal = {Bulletin of the American Mathematical Society},
	Number = {2},
	Pages = {255--308},
	Title = {Topology and data},
	Volume = {46},
	Year = {2009}}

@inproceedings{carlsson2004persistence,
	Author = {Carlsson, Gunnar and Zomorodian, Afra and Collins, Anne and Guibas, Leonidas},
	Booktitle = {Proceedings of the 2004 Eurographics/ACM SIGGRAPH symposium on Geometry processing},
	Pages = {124--135},
	Title = {Persistence barcodes for shapes},
	Year = {2004}}

@article{krishnan2020invertibility,
	Author = {Krishnan, Sanjeevi and Ogle, Crichton},
	Journal = {arXiv preprint arXiv:2010.11276},
	Title = {Invertibility in Category Representations},
	Year = {2020}}

@article{kocc2020representations,
	Author = {Ko{\c{c}}, Ayten and {\"O}zayd{\i}n, Murad},
	Journal = {Journal of pure and applied algebra},
	Number = {3},
	Pages = {1297--1319},
	Publisher = {Elsevier},
	Title = {Representations of Leavitt path algebras},
	Volume = {224},
	Year = {2020}}

@book{steinberg2016representation,
	Author = {Steinberg, Benjamin},
	Publisher = {Springer},
	Title = {Representation theory of finite monoids},
	Year = {2016}}

@article{patel2018generalized,
	Author = {Patel, Amit},
	Journal = {Journal of Applied and Computational Topology},
	Number = {3},
	Pages = {397--419},
	Publisher = {Springer},
	Title = {Generalized persistence diagrams},
	Volume = {1},
	Year = {2018}}

@article{alpert2021configuration,
	Author = {Alpert, Hannah and Manin, Fedor},
	Journal = {arXiv preprint arXiv:2107.04574},
	Title = {Configuration spaces of disks in a strip, twisted algebras, persistence, and other stories},
	Year = {2021}}

@article{carlsson2012computational,
	Author = {Carlsson, Gunnar and Gorham, Jackson and Kahle, Matthew and Mason, Jeremy},
	Journal = {Physical Review E},
	Number = {1},
	Pages = {011303},
	Publisher = {APS},
	Title = {Computational topology for configuration spaces of hard disks},
	Volume = {85},
	Year = {2012}}

@article{baryshnikov2014min,
	Author = {Baryshnikov, Yuliy and Bubenik, Peter and Kahle, Matthew},
	Journal = {International Mathematics Research Notices},
	Number = {9},
	Pages = {2577--2592},
	Publisher = {OUP},
	Title = {Min-type Morse theory for configuration spaces of hard spheres},
	Volume = {2014},
	Year = {2014}}

@article{Kahle2021configuration,
	Author = {Alpert, Hannah and Kahle, Matthew and MacPherson, Robert},
	Date-Modified = {2023-03-09 22:18:00 -0600},
	Journal = {Journal of Applied and Computational Topology},
	Number = {3},
	Pages = {357--390},
	Publisher = {Springer},
	Title = {Configuration spaces of disks in an infinite strip},
	Volume = {5},
	Year = {2021}}

@article{alpert2020configuration,
	Author = {Alpert, Hannah and Bauer, Ulrich and Kahle, Matthew and MacPherson, Robert and Spendlove, Kelly},
	Journal = {arXiv preprint arXiv:2010.14480},
	Title = {Configuration spaces of hard squares in a rectangle},
	Year = {2020}}

@article{nazarova1975partially,
	Author = {Nazarova, Lyudmila Aleksandrovna},
	Journal = {Mathematics of the USSR-Izvestiya},
	Number = {5},
	Pages = {911},
	Publisher = {IOP Publishing},
	Title = {Partially ordered sets of infinite type},
	Volume = {9},
	Year = {1975}}

@article{kleiner1972partially,
	Author = {Kleiner, MM},
	Journal = {Zapiski Nauchnykh Seminarov POMI},
	Pages = {32--41},
	Publisher = {St. Petersburg Department of Steklov Institute of Mathematics, Russian~{\ldots}},
	Title = {Partially ordered sets of finite type},
	Volume = {28},
	Year = {1972}}

@inproceedings{edelsbrunner2000topological,
	Author = {Edelsbrunner, Herbert and Letscher, David and Zomorodian, Afra},
	Booktitle = {Proceedings 41st annual symposium on foundations of computer science},
	Organization = {IEEE},
	Pages = {454--463},
	Title = {Topological persistence and simplification},
	Year = {2000}}


@article{skryzalin2017numeric,
	Author = {Skryzalin, Jacek and Carlsson, Gunnar},
	Journal = {Journal of Applied and Computational Topology},
	Number = {1},
	Pages = {89--119},
	Publisher = {Springer},
	Title = {Numeric invariants from multidimensional persistence},
	Volume = {1},
	Year = {2017}}

@inproceedings{carlsson2009computing,
	Author = {Carlsson, Gunnar and Singh, Gurjeet and Zomorodian, Afra},
	Booktitle = {International Symposium on Algorithms and Computation},
	Organization = {Springer},
	Pages = {730--739},
	Title = {Computing multidimensional persistence},
	Year = {2009}}

@inproceedings{robins1999towards,
	Author = {Robins, Vanessa},
	Booktitle = {Topology proceedings},
	Number = {1},
	Pages = {503--532},
	Title = {Towards computing homology from finite approximations},
	Volume = {24},
	Year = {1999}}

	
@article{asashiba2018interval,
  title={On interval decomposability of 2D persistence modules},
  author={Asashiba, Hideto and Buchet, Micka{\"e}l and Escolar, Emerson G and Nakashima, Ken and Yoshiwaki, Michio},
  journal={Computational Geometry},
  volume={105},
  pages={101879},
  year={2022},
  publisher={Elsevier}
}	
	
	

@article{botnan2022introduction,
	Author = {Botnan, Magnus Bakke and Lesnick, Michael},
	Journal = {arXiv preprint arXiv:2203.14289},
	Title = {An introduction to multiparameter persistence},
	Year = {2022}}

@article{lesnick2015interactive,
	Author = {Lesnick, Michael and Wright, Matthew},
	Journal = {arXiv preprint arXiv:1512.00180},
	Title = {Interactive visualization of 2-d persistence modules},
	Year = {2015}}

@article{lesnick2022computing,
	Author = {Lesnick, Michael and Wright, Matthew},
	Journal = {SIAM Journal on Applied Algebra and Geometry},
	Number = {2},
	Pages = {267--298},
	Publisher = {SIAM},
	Title = {Computing minimal presentations and bigraded betti numbers of 2-parameter persistent homology},
	Volume = {6},
	Year = {2022}}

@book{weibel1995introduction,
	Author = {Weibel, Charles A},
	Number = {38},
	Publisher = {Cambridge university press},
	Title = {An introduction to homological algebra},
	Year = {1995}}

@book{rotman2009introduction,
	Author = {Rotman, Joseph J},
	Publisher = {Springer},
	Title = {An introduction to homological algebra},
	Volume = {2},
	Year = {2009}}

@book{brown2012cohomology,
	Author = {Brown, Kenneth S},
	Publisher = {Springer Science \& Business Media},
	Title = {Cohomology of groups},
	Volume = {87},
	Year = {2012}}
	
@book{hatcher2002algebraic,
  title={Algebraic Topology},
  author={Hatcher, Allen},
  year={2002},
  publisher={Cambridge University Press}
}


==> chapters/chapter0.tex <==
\chapter{Introduction}




Topological data analysis (TDA) also provides a tool for understanding the shape of the data.


It was first inspired by the work of Marston Morse, followed by a sequence of pioneered papers, see for instance \cite{robins1999towards}\cite{ELZ} \cite{carlsson2004persistence}. The pipeline of TDA can be (roughly) described by three main steps:
\begin{itemize}
\item Obtaining the point cloud with a metric;
\item Constructing the geometric object (specifically, a filtered complex) from the point cloud with discrete or continuous parameters;
\item Calculating the homology groups of the filtered complex and the persistence diagram/barcode. Interpreting the topological and geometric features of the data via persistence diagram/barcode. 
\end{itemize} 
\begin{center}
\smartdiagramset{back arrow disabled=true}
\smartdiagram[flow diagram:horizontal]{Data,
 Filtered complex, Persistence diagram/ Barcode}
 \captionof{figure}{The pipeline of TDA}
\end{center}
 

One of the primary tasks in TDA is finding the proper representation (called 'barcode') of a given data cloud. The notion of barcodes is introduced in \cite{edelsbrunner2000topological}, and algorithms for computing barcodes of persistence modules are discovered by many researchers. Carlsson-Zomorodian (2015) studied the 1-dimensional persistence modules of finite type \cite{zomorodian2005computing}, that is, $(P,\leq)=(\mathbb{N},\leq)$ and each $M:(\mathbb{N},\leq)\rightarrow\mathsf{Vect}_{\mathbb{F}}$ has the property that $M_i$ is a finitely dimensional vector space for every $i\in\mathbb{N}$ and there exists $N\in\mathbb{N}$ such that morphism $M(i\leq i+1): M_i\rightarrow M_{i+1}$ is an isomorphism for all $i\geq N$. They proved that the category of persistence modules of finite type is equivalent to the category of finitely generated non-negatively graded $\mathbb{F}[x]$-modules. Using the equivalence of the categories, one can obtain an algebraic description of the barcode. Since $\mathbb{F}[x]$ is a principal ideal domain (PID), for each persistence module $M: (\mathbb{Z},\leq)\rightarrow \mathsf{vect}_{\mathbb{F}}$, there exists $m,n\in\mathbb{N}$ such that $$M\cong\left(\bigoplus\limits_{i=1}^{n}x^{a_i}\mathbb{F}[x]\right)\oplus\left(\bigoplus\limits_{j=1}^{m}x^{b_j}\mathbb{F}[x]/(x^{d_j})\right)$$ Therefore, the barcode of $M$ consists of the intervals $[a_i,\infty)$ for $i=1,\dots, n$ and $[b_j,d_j)$ for $j=1,\dots, m$. The ungraded version is the structure theorem for finitely generated modules over a PID, which is a standard result in commutative algebra.\\

%The following theorem gives the theoretical foundation of the barcodes of one-parameter pointwise finite-dimensional persistence modules:

%\begin{theorem}[Structure Theorem of Persistence Modules over a Totally Ordered Set\cite{crawley2015decomposition}]
%For a totally ordered set $T$ and pointwise finite-dimensional $T$-indexed persistence module $M$, there exists a unique multiset of intervals $B_M$ such that $$M\cong\bigoplus\limits_{I\in B_M}\mathbb{F}I$$
%where $\mathbb{F}I$ consists of
%$$\mathbb{F}I_t = \begin{cases} \mathbb{F}, & \mbox{if } t\in I\\ 0, & \mbox{if } t\notin I \end{cases} \mbox{ and } \Hom(\mathbb{F}I_t, \mathbb{F}I_s) = \begin{cases} \{id_{\mathbb{F}}\}, & \mbox{if } t\leq s\in I\\ 0, & \mbox{else} \end{cases} $$
%\end{theorem}
%The set $B_M$ is the barcode of the persistence module $M$, and $\mathbb{F}I$ is called the interval module with support on $I$. Interval modules are building blocks of 1-dimensional persistent modules. In particular, interval modules are indecomposable. The barcode representation contains the data cloud's algebraic and geometric features, and the data's shape can be understood using those features. For instance, the difference or similarity between the two data clouds can be evaluated by measuring the similarity of their barcodes.\\

Although the theory of $1$-dimensional TDA provides a powerful tool for helping people understand data, the data cloud itself may naturally come with more than one parameter. Analyzing one parameter at a time is time-consuming and can be information-losing: it only contains a slice of the feature by fixing all but one parameter. On the other hand, the data cloud may contain noise. By considering the density of the data as a parameter along with the radius parameter, one can remove the noise from the data accordingly and analyze the shape of the data at various density levels.\\ 

Multi-parameter topological data analysis has promising application potential in dealing with higher-dimensional data clouds and data clouds with noise, and the theory of multi-parameter TDA is growing. One significant difficulty in the multi-parameter persistence theory is that there is no canonical way to define the higher-dimensional barcodes (which represent indecomposable representations) analogous to the one-dimension barcodes because there is no structure theorem available in $\mathsf{vect}_{\mathbb{F}}^{(P,\leq)}$ when the poset $P$ is not a totally ordered set. For example, it is impossible to classify the indecomposable representations of $2$-parameter persistence modules. Every point-wise finite-dimensional $2$-parameter persistence module corresponds to a finitely generated $\mathbb{Z}^2$-graded module over $\mathbb{F}[x,y]$, up to isomorphism, but there is no classification theorem of finitely generated $\mathbb{Z}^2$-graded modules over $\mathbb{F}[x,y]$. Consequently, the indecomposable submodules of a multidimensional persistence module can be very complicated. Buchet-Escolar shows that any n-dimensional persistence module can be embedded as a slice of an indecomposable (n+1)-parameter persistence module\cite{BE-2020}\cite{BE-2019}, that is, for every $n$-parameter persistence module $M$, there exists an indecomposable $(n+1)$-parameter persistence module $N$ such that $M=N\circ \iota$, where $\iota:(\mathbb{Z}^n,\leq)\rightarrow (\mathbb{Z}^{n+1},\leq)$ is a functor that is injective on objects. 



%An algorithm for finding generators of a zigzag persistence module was discovered by Gunnar Carlsson, Anjan Dwaraknath and Bradley J. Nelson in their paper \cite{2021}. Algorithms for finding generators of an interval-decomposable 2-dimensional persistence module are known, cf.\cite{asashiba2018interval} and an algorithm for finding minimal presentations and bigraded Betti numbers of a 2-dimensional persistence module when it is not necessarily interval-decomposable is provided in \cite{lesnick2022computing}.\\


%It is well-known that polytope modules are thin and indecomposable. See Lemma \ref{thinpoly}. In Section \ref{TPM}, we proved that the converse is true in $\mathbb{R}^2$, up to isomorphism. 
%\begin{theorem}
%Every indecomposable thin persistence module $M\in\cat{vect}_{\mathbb{F}}^{(\mathbb{R}^2, \leq)}$ is isomorphic to a polytope module.
%\end{theorem}


In this thesis, we want to apply the multi-parameter TDA theory to understand complicated geometric objects. In particular, we want to understand how the configuration spaces change along with the changes in the proximity conditions. In 2013, Dover-\"Ozayd\i n studied the restricted configuration space of metric graphs and gave an upper bound for the number of homeomorphism types of its $n$-th configuration space over proximity conditions.\cite{dover2013homeomorphism} As a continuation of their pioneering work, we study the multi-parameter persistence modules given by the filtrations of the $n$-th configuration spaces (with two restraint parameters) of finite metric graphs. In addition to the parameters representing the minimum distance allowed between each pair of robots, we also consider the parameters representing the length of edges (denoted by $\mathbf{L}$). Therefore, for a metric graph $\Gamma=(V,E)$, the n-th configuration space with restraint parameter $\mathbf{r}\in \mathbb{R}_{\geq 0}^{\binom{n}{2}}$ and edge length parameter $\mathbf{L}=(L_e)_{e\in E}\in \mathbb{R}_{\geq 0}^{\lvert E\rvert}$ is 
$$X^{n}_{\mathbf{r},\mathbf{L}}=\{(x_{1},\dots, x_{n})\in X^{n}\mid \delta(x_{i},x_{j})\geq r_{ij}, i,j=1,\dots, n, \mbox{ and } k=1,\dots, \lvert E\rvert\}$$
The object that we are investigating is a filtration of the spaces $\{X^{n}_{\mathbf{r},\mathbf{L}}\}$. This filtration naturally comes with ${\binom{n}{2}}+\lvert E\rvert$ parameters \cite{dover2013homeomorphism}. In particular, when all robots have the same size and all edges have fixed lengths, the problem reduces to a single-parameter problem, and one can apply the (single-parameter) TDA theory to analyze the filtration of configuration spaces. %One essential property the "higher dimensional barcodes" should have is that the intersection of it with any one-dimensional affine subspace of parameter space is a barcode. \\

In Section \ref{2ex}, we discuss an example which motivates this thesis.\\
\section{First Example}\label{2ex}
Let Y be a metric graph with the shape of $Y$ with the following metric: two edges of Y have length $1$, and the length of the other edge (labeled by $e_1$) varies. Let $e_2$ and $e_3$ denote the other two edges of $Y$. In this example, we interpret the metric graph $Y$ as a $Y$-shaped rail and consider two distinct thick robots (denoted by red robot and green robot) moving on $Y$, see figure \ref{Y2}. Let $r$ denote the minimum distance required between the two robots and let $L_{e_1}$ denote the length of the edge $e_1$. We denote its configuration space by $Y^2_{r,L_{e_1}}$. 
\begin{figure}[htbp!]
\centering
%\begin{minipage}{0.5\textwidth}
\resizebox{3.5cm}{!}{
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Straight Lines [id:da2635781359540772] 
\draw [line width=2.25]    (147.42,58.58) -- (102.5,103.5) ;
%Shape: Circle [id:dp7910752585821121] 
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 150 }  ,fill opacity=1 ] (127,72.75) .. controls (127,69.3) and (129.8,66.5) .. (133.25,66.5) .. controls (136.7,66.5) and (139.5,69.3) .. (139.5,72.75) .. controls (139.5,76.2) and (136.7,79) .. (133.25,79) .. controls (129.8,79) and (127,76.2) .. (127,72.75) -- cycle ;
%Straight Lines [id:da6907052067844686] 
\draw [line width=2.25]    (67,68.5) -- (102.5,103.5) ;
%Straight Lines [id:da520623802713565] 
\draw [line width=2.25]    (102.5,103.5) -- (102.5,161.58) ;
%Shape: Circle [id:dp3388574585166113] 
\draw  [fill={rgb, 255:red, 255; green, 16; blue, 0 }  ,fill opacity=1 ] (79,87.25) .. controls (79,83.8) and (81.8,81) .. (85.25,81) .. controls (88.7,81) and (91.5,83.8) .. (91.5,87.25) .. controls (91.5,90.7) and (88.7,93.5) .. (85.25,93.5) .. controls (81.8,93.5) and (79,90.7) .. (79,87.25) -- cycle ;
%Straight Lines [id:da048432554697130925] 
\draw [line width=2.25]  [dash pattern={on 2.53pt off 3.02pt}]  (48,49.5) -- (67,68.5) ;

% Text Node
\draw (45,68) node [anchor=north west][inner sep=0.75pt]   [align=left] {$e_1$};
% Text Node
\draw (109,136) node [anchor=north west][inner sep=0.75pt]   [align=left] {$e_2$};
% Text Node
\draw (152,53) node [anchor=north west][inner sep=0.75pt]   [align=left] {$e_3$};
% Text Node
\draw (72,93) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 255; green, 16; blue, 0}  ,opacity=1 ] [align=left] {$x$};
% Text Node
\draw (138.25,75.75) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 126; green, 201; blue, 100 }  ,opacity=1 ] [align=left] {$y$};
\end{tikzpicture}
}
\captionof{figure}{}
\label{Y2}
%\label{fig:fig3}  
%\caption{$Y^{\underline{2}}$: Second configuration space of $Y$ (all edges have length $1$)}
\end{figure}%



One cell of $Y^2_{r,L_{e_1}}$ is given by (\ref{9}).\\ 

\noindent\begin{minipage}{0.45\linewidth}
\begin{equation}\label{9}
\begin{aligned}
0&\leq x\leq 1=L_{e_2}\\
0&\leq y\leq 1=L_{e_3}\\
x&+y\geq r
\end{aligned}
\end{equation}
\end{minipage}%
\begin{minipage}{0.45\linewidth}
\begin{equation}\label{9'}
\begin{aligned}
0&\leq x\leq 1=L_{e_3}\\
0&\leq y\leq 1=L_{e_2}\\
x&+y\geq r
\end{aligned}
\end{equation}
\end{minipage}

\vspace{0.5cm}
The system of inequalities (\ref{9}) corresponds to the case when the red robot is on edge $e_2$ and the green robot is on edge $e_3$, while the system of inequalities (\ref{9'}) corresponds to the case when the red robot is on edge $e_3$ and the green robot is on edge $e_2$. \\

Similarly, the system of inequalities (\ref{10}) (\ref{11}) (\ref{12}) gives 2-dimensional cells of $Y^2_{r,L_{e_1}}$: for $i=2,3$,\\

\noindent\begin{minipage}{0.33\linewidth}
    \begin{equation}\label{10}
\begin{aligned}
0&\leq x_1\leq L_{e_1}\\
0&\leq x_2\leq 1=L_{e_i}\\
x_1&+x_2\geq r
\end{aligned}
\end{equation}
\end{minipage}%
\begin{minipage}{0.33\linewidth}
    \begin{equation}\label{11}
\begin{aligned}
0&\leq x_1\leq  1=L_{e_i}\\
0&\leq x_2\leq L_{e_1}\\
x_1&+x_2\geq r
\end{aligned}
\end{equation}
\end{minipage}%
\begin{minipage}{0.33\linewidth}
 \begin{equation}\label{12}
\begin{aligned}
0&\leq x_1\leq L_{e_1}\\
0&\leq x_2\leq L_{e_1}\\
x_1&+x_2\geq r
\end{aligned}
\end{equation}
\end{minipage}

\vspace{0.5cm}
There is another type of 2-dimensional cells in $Y^2_{r,L_{e_1}}$ and those cells correspond to the case when the red robot and green robot are on the same edge of $Y$: for $i=1,2,3$, \\

\noindent\begin{minipage}{0.45\linewidth}
\begin{equation}\label{14}
\begin{aligned}
0&\leq x\leq 1=L_{e_i}\\
0&\leq y\leq 1=L_{e_i}\\
x&-y\geq r
\end{aligned}
\end{equation}
\end{minipage}%
\begin{minipage}{0.45\linewidth}
\begin{equation}\label{14'}
\begin{aligned}
0&\leq x\leq 1=L_{e_i}\\
0&\leq y\leq 1=L_{e_i}\\
y&-x\geq r
\end{aligned}
\end{equation}
\end{minipage}

\vspace{0.5cm}
The system of inequalities (\ref{14}) corresponds to the case when the distance between the red robot and the center of $Y$ is greater than the distance between the green robot and the center of $Y$, while the system of inequalities (\ref{14'}) corresponds to the opposite scenario. Note that the critical hyperplanes are 
 \begin{equation}\label{15}
\begin{aligned}
r_{12}&=1\\
r_{12}&=2\\
r_{12}&=L_{e_1}\\
r_{12}&=L_{e_1}+1
\end{aligned}
\end{equation}
We then obtain the hyperplane arrangement in the parameter space where each point $(r,L_{e_1})$ in the hyperplane corresponds to a restricted configuration space $Y^2_{r,L_{e_1}}$, as shown in figure \ref{para0}. Note that $Y^2_{r_1,l_1}$ and $Y^2_{r_2,l_2}$ are homotopy equivalent (or even stronger, isotopy equivalent) when the points $(r_1,l_1)$ and $(r_2,l_2)$ are contained in the same chamber.\\

\noindent\begin{minipage}[c]{0.45\textwidth}
\centering
\resizebox{5cm}{!}{


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,980); %set diagram left start at 0, and has height of 980

%Shape: Polygon [id:ds11506870492607946] 
\draw  [draw opacity=0][fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.4 ] (138.9,52.47) -- (237.3,51.32) -- (236.79,104.89) -- (139.57,203.47) -- (138.9,106.03) -- cycle ;
%Shape: Right Triangle [id:dp6201655647143911] 
\draw  [draw opacity=0][fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.4 ] (138.76,203.83) -- (235.65,106.03) -- (236.05,203.42) -- cycle ;
%Shape: Axis 2D [id:dp9731816624191663] 
\draw  (6.75,299.04) -- (373.46,299.04)(43.42,46.75) -- (43.42,327.07) (366.46,294.04) -- (373.46,299.04) -- (366.46,304.04) (38.42,53.75) -- (43.42,46.75) -- (48.42,53.75)  ;
%Shape: Right Triangle [id:dp4928494811939903] 
\draw  [draw opacity=0][fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.4 ] (43.42,299.04) -- (139.57,203.47) -- (139.82,298.78) -- cycle ;
%Shape: Right Triangle [id:dp9769707308506641] 
\draw  [draw opacity=0][fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.4 ] (139.82,298.78) -- (235.28,202.82) -- (235.53,298.53) -- cycle ;
%Shape: Right Triangle [id:dp5096030264480254] 
\draw  [draw opacity=0][fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.4 ] (289.7,50.84) -- (236.79,104.89) -- (236.25,51.39) -- cycle ;
%Shape: Right Triangle [id:dp08599477187888893] 
\draw  [draw opacity=0][fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.4 ] (331.68,106.33) -- (234.91,204.42) -- (235.48,105.78) -- cycle ;
%Shape: Polygon [id:ds3392647219241056] 
\draw  [draw opacity=0][fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.4 ] (289.7,50.7) -- (386.49,51.53) -- (330.94,106.22) -- (331.68,106.33) -- (313,106) -- (234.5,105.89) -- cycle ;
%Shape: Polygon [id:ds7330989816504343] 
\draw  [draw opacity=0][fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.4 ] (138.9,52.47) -- (138.9,106.03) -- (139.57,203.47) -- (43.42,299.04) -- (43.93,52.47) -- cycle ;
%Shape: Right Triangle [id:dp4636151324255011] 
\draw  [draw opacity=0][fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.4 ] (236.88,203.18) -- (140.21,298.72) -- (139.58,203.82) -- cycle ;
%Straight Lines [id:da3168733776934405] 
\draw [line width=1.5]    (43.42,299.04) -- (289.7,50.84) ;
%Straight Lines [id:da08247699052421664] 
\draw [line width=1.5]    (140.21,299.72) -- (386.49,51.53) ;
%Straight Lines [id:da9751424588701745] 
\draw [line width=1.5]    (140.21,299.72) -- (138.9,52.47) ;
%Straight Lines [id:da0007968547538703685] 
\draw [line width=1.5]    (235.53,298.53) -- (234.22,51.28) ;

% Text Node
\draw (139.47,313.34) node   [align=left] {1};
% Text Node
\draw (236.73,312.19) node   [align=left] {2};
% Text Node
\draw (35.35,203.5) node   [align=left] {1};
% Text Node
\draw (34.21,108.53) node   [align=left] {2};
% Text Node
\draw (17.07,17.96) node [anchor=north west][inner sep=0.75pt]    {$L_{e_{1}}$};
% Text Node
\draw (376.76,302.52) node [anchor=north west][inner sep=0.75pt]    {$r_{12}$};


\end{tikzpicture}
}
\captionof{figure}{The hyperplane arrangement of $\mathbb{R}^2$ associated to $Y^2_{r,L_{e_1}}$}
\label{para0}
\end{minipage}
\noindent\begin{minipage}[c]{0.45\textwidth}
\centering
\resizebox{5cm}{!}{


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,365); %set diagram left start at 0, and has height of 365

%Shape: Polygon [id:ds04142214750274431] 
\draw  [draw opacity=0][fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ] (122.5,32) -- (208.5,31) -- (206.05,77.81) -- (121.38,163.29) -- (123.5,78) -- cycle ;
%Shape: Right Triangle [id:dp597542485421235] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (121.38,163.29) -- (206.05,77.81) -- (206.41,162.93) -- cycle ;
%Shape: Rectangle [id:dp9264199893981724] 
\draw  [draw opacity=0][fill={rgb, 255:red, 80; green, 227; blue, 194 }  ,fill opacity=1 ] (39.43,32) -- (122.5,32) -- (122.5,164.79) -- (39.43,164.79) -- cycle ;
%Shape: Right Triangle [id:dp010769941557449814] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (207.11,163.12) -- (122.94,249.09) -- (122.08,163.98) -- cycle ;
%Shape: Right Triangle [id:dp9998752781882319] 
\draw  [fill={rgb, 255:red, 80; green, 227; blue, 194 }  ,fill opacity=1 ] (123.73,163.79) -- (39.56,249.77) -- (38.7,164.65) -- cycle ;
%Shape: Axis 2D [id:dp13002815456038697] 
\draw  (7,247.5) -- (327.5,247.5)(39.05,27) -- (39.05,272) (320.5,242.5) -- (327.5,247.5) -- (320.5,252.5) (34.05,34) -- (39.05,27) -- (44.05,34)  ;
%Shape: Square [id:dp12226237677297158] 
\draw   (39.43,80) -- (207.06,80) -- (207.06,247.63) -- (39.43,247.63) -- cycle ;
%Shape: Right Triangle [id:dp7453048669112339] 
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ] (39.82,247.68) -- (123.25,163.81) -- (123.46,247.46) -- cycle ;
%Straight Lines [id:da48460316293413275] 
\draw    (39.43,247.63) -- (123.08,163.98) ;
%Straight Lines [id:da750216453119956] 
\draw    (122.5,31) -- (122.68,247.29) ;
%Straight Lines [id:da12428539346664969] 
\draw    (38.7,163.65) -- (207.46,164.31) ;
%Shape: Circle [id:dp27859721078429556] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (359.53,158.82) .. controls (359.53,155.51) and (362.21,152.82) .. (365.53,152.82) .. controls (368.84,152.82) and (371.53,155.51) .. (371.53,158.82) .. controls (371.53,162.14) and (368.84,164.83) .. (365.53,164.83) .. controls (362.21,164.83) and (359.53,162.14) .. (359.53,158.82) -- cycle ;
%Shape: Circle [id:dp1438504635106319] 
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ] (360.5,199.83) .. controls (360.5,196.51) and (363.19,193.83) .. (366.5,193.83) .. controls (369.81,193.83) and (372.5,196.51) .. (372.5,199.83) .. controls (372.5,203.14) and (369.81,205.83) .. (366.5,205.83) .. controls (363.19,205.83) and (360.5,203.14) .. (360.5,199.83) -- cycle ;
%Shape: Circle [id:dp821374354647445] 
\draw  [fill={rgb, 255:red, 80; green, 227; blue, 194 }  ,fill opacity=1 ] (360.38,179.83) .. controls (360.38,176.51) and (363.06,173.83) .. (366.38,173.83) .. controls (369.69,173.83) and (372.38,176.51) .. (372.38,179.83) .. controls (372.38,183.14) and (369.69,185.83) .. (366.38,185.83) .. controls (363.06,185.83) and (360.38,183.14) .. (360.38,179.83) -- cycle ;
%Shape: Circle [id:dp39853861632643883] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ] (361.38,221.83) .. controls (361.38,218.51) and (364.06,215.83) .. (367.38,215.83) .. controls (370.69,215.83) and (373.38,218.51) .. (373.38,221.83) .. controls (373.38,225.14) and (370.69,227.83) .. (367.38,227.83) .. controls (364.06,227.83) and (361.38,225.14) .. (361.38,221.83) -- cycle ;
%Shape: Right Triangle [id:dp3146204215957056] 
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ] (123.68,246.99) -- (207.11,163.12) -- (207.33,246.77) -- cycle ;
%Straight Lines [id:da101770580921972] 
\draw    (207.5,26) -- (207.06,247.63) ;
%Shape: Right Triangle [id:dp8014171959942671] 
\draw  [draw opacity=0][fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ] (254.29,29.58) -- (208.05,76.81) -- (207.58,30.06) -- cycle ;
%Shape: Right Triangle [id:dp25863626758292346] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ] (290.34,78.11) -- (207.11,163.12) -- (206.26,78.96) -- cycle ;
%Shape: Polygon [id:ds5999221723066952] 
\draw  [draw opacity=0][fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ] (254.29,29.58) -- (333.5,27) -- (290.34,78.11) -- (290.34,78.11) -- (206.05,77.81) -- cycle ;

% Text Node
\draw (334,263) node   [align=left] {$r_{12}$};
% Text Node
\draw (31,12) node   [align=left] {$L_{e_1}$};
% Text Node
\draw (405,160.27) node   [align=left] {6 points};
% Text Node
\draw (406,200.27) node   [align=left] {2 points};
% Text Node
\draw (403,180.27) node   [align=left] {1 circle};
% Text Node
\draw (407,222.27) node   [align=left] {4 points};
% Text Node
\draw (123,260) node   [align=left] {1};
% Text Node
\draw (208,259) node   [align=left] {2};
% Text Node
\draw (32,164) node   [align=left] {1};
% Text Node
\draw (31,81) node   [align=left] {2};


\end{tikzpicture}
}
\captionof{figure}{Homotopy type of $Y^2_{r,L_{e_1}}$}
\label{chap1:para}
\end{minipage}

We want to understand how much the space will change if we perturb the parameters. For example, when $L_{e_1}=1$, the space $Y^2_{r,1}$ changes as $r$ goes from $0$ to $2$:  \\

\input{fig13}

Now we consider $Y^2_{r,2}$ with $r$ varies. In other words, we consider the restricted configuration spaces of $Y$ when the length of edge $e_1$ is $2$. Figure \ref{fig:14-}- \ref{fig:18} illustrate the changes of $Y^2_{r,1}$ as $r$ goes from $0$ to $2$:\\

\input{fig14}

The homotopy type of $Y^2_{r,L_{e_1}}$ for each $r$ and $L_{e_1}$ is given in Figure \ref{chap1:para}. We want to understand the $2$-parameter persistence module $PH_i(Y^2_{\mathbf{r},2};\mathbb{F})$. In particular, we want to answer the following questions:
\begin{itemize}
\item Is $PH_i(Y^2_{\mathbf{r},2};\mathbb{F})$ interval indecomposable?
\item What are the indecomposable direct summands of $PH_i(Y^2_{\mathbf{r},2};\mathbb{F})$? 
\end{itemize}





==> chapters/section1.05.tex <==
\section{Graphs}

A \textbf{directed graph} (also called \textbf{digraph} or \textbf{quiver})  $Q=(V,E,s,t)$ consists of two sets $V$ (called the set of vertices) and $E$ (called the set of arrows), and two maps $s,t: E\rightarrow V$ where $s$ sends each edge to its source, and $t$ sends each edge to its target. $Q=(V,E,s,t)$ is said to be \textbf{finite} if $V$ and $E$ are finite sets. $Q=(V,E,s,t)$ is said to be \textbf{connected} (as a digraph) if there is a directed path between any two vertices of $Q$. We can view a quiver $Q=(V,E,s,t)$ as a category where $V$ is the set of objects and the set of morphisms consists of all the paths in $Q$. \\


A \textbf{graph}\index{graph} $\Gamma=(V,E,\mathrm{I}_{\Gamma})$ consists of two sets $V$ (called the set of vertices) and $E$ (called the set of edges), and a function represent the incidence relation: $\mathrm{I}_{\Gamma}: E\rightarrow V^{[2]}$ where $V^{[2]}$ is the collection of subsets of $V$ with cardinality $2$. When $V$ and $E$ are finite sets, we call $\Gamma$ a \textbf{finite graph}.\\

\textcolor{red}{
Given two graphs $\Gamma=(V,E,\mathrm{I}_{\Gamma})$ and $\Gamma'=(V',E',\mathrm{I}_{\Gamma'})$, a \textbf{graph morphism} $f$ from $\Gamma$ to $\Gamma'$ is a pair of maps $f_V:V\rightarrow V'$ and $f_E:E\rightarrow E'$ such that $\mathrm{I}_{\Gamma'}(f_E(e))\subseteq f^\ast_V(\mathrm{I}_{\Gamma}(e))$ where $f^{\ast}_V: V^{[2]}\rightarrow V'^{[2]}$ is defined as $f^{\ast}_V(S)=\{f_V(s)\mid s\in S\}$.
The category of graphs, denoted by $\cat{Graph}$, has graphs as its objects and graph morphisms as its morphisms. A full subcategory that consists of finite graphs is denoted by $\cat{FinGraph}$.\\
}

A \textbf{tree}\index{tree} is a connected graph with no loops or cycles. A \textbf{star graph}\index{star graph} with $k$ leaves is a tree with $k+1$ vertices and $k$ edges such that there is exactly one vertex has degree $k$ and the degree of the other vertices is $1$. 
\begin{figure}[htbp!]
\centering
\resizebox{3.5cm}{!}{

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Straight Lines [id:da972900764614677] 
\draw    (100,113) -- (66,61.5) ;
\draw [shift={(66,61.5)}, rotate = 236.57] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(100,113)}, rotate = 236.57] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da6593634943583064] 
\draw    (100,113) -- (127,55.5) ;
\draw [shift={(127,55.5)}, rotate = 295.15] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da19483909403171662] 
\draw    (100,113) -- (163,113) ;
\draw [shift={(163,113)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(100,113)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da5399503195257365] 
\draw    (43,127.5) -- (100,113) ;
\draw [shift={(100,113)}, rotate = 345.73] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(43,127.5)}, rotate = 345.73] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da5048914562679376] 
\draw    (72,175) -- (100,113) ;
\draw [shift={(100,113)}, rotate = 294.3] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(72,175)}, rotate = 294.3] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da46171788233588984] 
\draw    (146,158.5) -- (100,113) ;
\draw [shift={(100,113)}, rotate = 224.69] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(146,158.5)}, rotate = 224.69] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;

% Text Node
\draw (96.73,159.77) node [anchor=north west][inner sep=0.75pt]  [font=\Large,rotate=-347.31] [align=left] {...};
% Text Node
\draw (169,105) node [anchor=north west][inner sep=0.75pt]   [align=left] {1};
% Text Node
\draw (128,35) node [anchor=north west][inner sep=0.75pt]   [align=left] {2};
% Text Node
\draw (148,161.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {k};
% Text Node
\draw (54,42) node [anchor=north west][inner sep=0.75pt]   [align=left] {3};
% Text Node
\draw (28,122) node [anchor=north west][inner sep=0.75pt]   [align=left] {4};
% Text Node
\draw (61,178) node [anchor=north west][inner sep=0.75pt]   [align=left] {5};


\end{tikzpicture}}
\caption{$\mathrm{Star}_k$}
\label{fig:4a}
\end{figure}

\section{Posets, Pomonoids, and Cayley Graphs}
Let $(P,\leq)$ be a poset. A subposet $\cat{I}$ of $(P,\leq)$ is \textbf{connected} if for every $x,y\in \cat{I}$, there exists $z_1,\dots, z_n\in I$ for some $n$ such that one of the following is true:
\begin{list}{$\diamond$}{}  
\item $x\leq z_1\geq z_2\leq \cdots \leq z_n\geq y$
\item $x\leq z_1\geq z_2\leq \cdots \geq z_n\leq y$
\item $x\geq z_1\leq z_2\leq \cdots \leq z_n\geq y$
\item $x\geq z_1\leq z_2\leq \cdots \geq z_n\leq y$
\end{list}
$\cat{I}$ is \textbf{convex} if for every $x\leq z\leq y\in P$, $x,y\in \cat{I}$ implies $z\in \cat{I}$.
$(P,\leq)$ is locally-finite if there are only finitely many elements between $x$ and $y$ for all $x,y\in P$.
\begin{definition}[Interval of a poset]
$\cat{I}\subseteq (P,\leq)$. $\cat{I}$ is called an \textbf{interval}\index{interval} if it is convex and connected.
\end{definition}

A poset $(P,\leq)$ is \textbf{bounded}\index{bounded poset} if $P$ contains an initial element and a terminal element as a category. $(P,\leq)$ has \textbf{finite height}\index{height of a poset} if the length of the maximal chains from $x$ to $y$ is bounded for all $x,y\in P$. A bounded poset $(P,\leq)$ is \textbf{graded}\index{graded poset} if $(P,\leq)$ has finite height and all maximal chains of $P$ have the same length.


\begin{definition}\label{Lposet}\index{edge-labeled poset}
Let $(P,\leq)$ be a graded and bounded poset. $(P,\leq)$ is \textbf{edge-labeled} by a set $S$ if every covering relation of $(P,\leq)$ is labeled by an element of $S$.
\end{definition}

\begin{definition}\label{Group_poset}\index{pomomoid}
Let $(P,\leq)$ be an edge-labeled poset by a set $S$. Then a monoid $M(P)$ is the quotient monoid of the free monoid $\langle S\rangle$ subject to a congruence relation $amb\sim am'b$ for any maximal chains $m, m'$ of $(P,\leq)$ and $a,b\in\langle S\rangle$. There is a natural partial order on $\langle S\rangle$: $a\leq b\in \langle S\rangle$ if and only if there exists $s\in \langle S\rangle$ such that $b=as$. A partial order on $M(P)$ is inherited from $\langle S\rangle$: $\bar{a}\leq \bar{b}\in M(P)$ if and only if there exists $\bar{s}\in M(P)$ such that $\bar{b}=\bar{a}\bar{s}$. We call the poset $M(P)$ with the inherited partial order from $\langle S\rangle$ the pomonoid generated by $S$, and denoted this poset by $(M(P), \leq_S)$.
\end{definition}


\begin{definition}\label{CayleyGraph}\index{Cayley graph}
Let $G$ be a group and $S$ be a subset of $G$. The (right) \textbf{Cayley graph} of $G$ by $S$, denoted by $\textsc{Cayley}(G,S)$, is a vertex-labeled directed graph where each vertex is labeled by a word of $G$, and two vertices $x$ and $y$ of $\textsc{Cayley}(G,S)$ are connected by an arrow from $x$ to $y$ if there exists $s\in S$ such that $y=xs$.
\end{definition}






==> chapters/section1.5.tex <==
\section{Quiver Representations}

\begin{definition}\index{quiver representation}
Let $Q$ be a quiver (viewed as a category). A \textbf{quiver representation} over the quiver $Q$ is a functor $M: Q\rightarrow \cat{Vect}_{\mathbb{F}}$. 
\end{definition}

\begin{definition}\index{thin representation}
Let $M$ be a quiver representation over the quiver $Q$. Then $M$ is \textbf{thin} if $\dim Mv\leq 1$ for all $v\in\ob Q$. 
\end{definition}

Let $\mathbb{A}_n$ denote the quivers whose underlying graph is \\
\begin{figure}[bthp!]
\centering
        \resizebox{8cm}{!}{


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Straight Lines [id:da48014859020204725] 
\draw    (14,43.7) -- (80.83,43.7) ;
\draw [shift={(80.83,43.7)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(14,43.7)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da8699773493822802] 
\draw    (80.83,43.7) -- (147.65,43.7) ;
\draw [shift={(147.65,43.7)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(80.83,43.7)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da2887142658719948] 
\draw    (147.65,43.7) -- (187.25,43.7) ;
\draw [shift={(147.65,43.7)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da5729232584571307] 
\draw    (241.7,43.7) -- (280.06,43.7) ;
\draw [shift={(280.06,43.7)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da513801377645944] 
\draw    (280.06,43.7) -- (346.89,43.7) ;
\draw [shift={(346.89,43.7)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(280.06,43.7)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da6247434048579639] 
\draw    (346.89,43.7) -- (413.71,43.7) ;
\draw [shift={(413.71,43.7)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(346.89,43.7)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da7070410051785767] 
\draw    (203.71,43.7) ;
\draw [shift={(203.71,43.7)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 1.34, y radius= 1.34]   ;
\draw [shift={(203.71,43.7)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 1.34, y radius= 1.34]   ;
%Straight Lines [id:da06968311942087024] 
\draw    (211,43.7) ;
\draw [shift={(211,43.7)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 1.34, y radius= 1.34]   ;
\draw [shift={(211,43.7)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 1.34, y radius= 1.34]   ;
%Straight Lines [id:da20479773593908268] 
\draw    (219,43.7) ;
\draw [shift={(219,43.7)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 1.34, y radius= 1.34]   ;
\draw [shift={(219,43.7)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 1.34, y radius= 1.34]   ;




\end{tikzpicture}    
}
\end{figure}

where the graph has $n$ vertices.
\begin{theorem}\label{An}
Any representation of a type $\mathbb{A}_n$ quiver is a direct sum of thin indecomposable representations.
\end{theorem}
The converse of Theorem \ref{An} is true as well.
\begin{theorem}\label{AnConv}
Let $Q$ be a finite connect quiver. If every indecomposable representation of the quiver $Q$ is thin, then $Q$ is a type $\mathbb{A}_n$ quiver.
\end{theorem}

\paragraph{Admissible ideals and quotients of path algebras}
Let $\Gamma=(V,E,s,t)$ be a finite quiver and $k\Gamma$ be the path algebra of $\Gamma$. An \textbf{arrow ideal} $R_{\Gamma}$ of $k\Gamma$ is a two-sided ideal generated by the arrows of $\Gamma$. $R_{\Gamma}$ has a natural $\mathbb{N}$-grading: $$R_{\Gamma}\cong\bigoplus\limits_{i=1}^{\infty}k\Gamma_i$$ where $\Gamma_i$ is the set of paths of $\Gamma$ which have length $i$. We use $R_{\Gamma}^m$ to denote the subalgebra of $R_{\Gamma}$ generated by all paths of length greater or equal to $m$:
$$R_{\Gamma}^m\cong\bigoplus\limits_{i=m}^{\infty}k\Gamma_i$$
It is clear that $R_{\Gamma}\supseteq R_{\Gamma}^2\supseteq R_{\Gamma}^3\supseteq R_{\Gamma}^4\supseteq \cdots \supseteq R_{\Gamma}^m\supseteq \cdots$
\begin{definition}
A two-sided ideal $I$ of $k\Gamma$ is an \textbf{admissible ideal} if there exists an integer $m\geq 1$ such that $$R_{\Gamma}^m\supseteq I \supseteq R_{\Gamma}^2$$
\end{definition}
\begin{example}
Let $\Gamma=(V,E,s,t)$ be a finite quiver and $a,b,c,d\in E$. Let $I_1$ be the ideal of $k\Gamma$ generated by $ab-cd$ and $I_2$ be the ideal of $k\Gamma$ generated by $ab-c$. Then $I_1$ is an admissible ideal while $I_2$ is not. 
\end{example}
\begin{proposition}\label{prop:pos}
Let $\Gamma$ be a finite digraph that has a full subgraph isomorphic to 
\begin{figure}[bthp!]
\centering
        \resizebox{2.5cm}{!}{


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Straight Lines [id:da6649514814486872] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (42,28) -- (96,78) ;
\draw [shift={(96,78)}, rotate = 42.8] [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(64.23,48.58)}, rotate = 42.8] [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(42,28)}, rotate = 42.8] [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da19350167630245085] 
\draw    (96,28) -- (96,78) ;
\draw [shift={(96,78)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(96,46.5)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(96,28)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da48014859020204725] 
\draw    (42,28) -- (96,28) ;
\draw [shift={(96,28)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(62.5,28)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(42,28)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;

% Text Node
\draw (56,55.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$c$};
% Text Node
\draw (64,5.4) node [anchor=north west][inner sep=0.75pt]    {$a$};
% Text Node
\draw (105,41.4) node [anchor=north west][inner sep=0.75pt]    {$b$};


\end{tikzpicture}
}
\end{figure}

Let $\tilde{\Gamma}$ be a subgraph of $\Gamma$, deleting the edge $c$. Then $\mathbb{F}\Gamma/(c-ba)\cong \mathbb{F}\tilde{\Gamma}$.
\end{proposition}
\begin{proof}
Define $\Phi:\mathbb{F}\Gamma\rightarrow \mathbb{F}\tilde{\Gamma}$ as follows: for all $d\in E$, $$\Phi(d)=\begin{cases} d, & \mbox{if } d\neq c\\ ba, & \mbox{if } d=c\end{cases}$$
Extend $\Phi$ to be an $\mathbb{F}$-algebra homomorphism. By the construction of $\Phi$, $\Phi$ is surjective. Note that $\ker(\Phi)=\{(\sum\alpha_{ij}p_i(c-ba)p_j\mid\alpha_i \in \mathbb{F}, p_i, p_j \mbox{ are paths of } \Gamma\}=(c-ba)$, hence $\mathbb{F}\Gamma/(c-ba)\cong \mathbb{F}\tilde{\Gamma}$.
\end{proof}

\begin{example}
Consider the quiver $P$ given by the figure below, where each triangle of the diagram is commutative: 
\begin{figure}[bthp!]
\centering
        \resizebox{4cm}{!}{
   

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Straight Lines [id:da6649514814486872] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (22,25) -- (76,75) ;
\draw [shift={(76,75)}, rotate = 42.8] [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(44.23,45.58)}, rotate = 42.8] [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(22,25)}, rotate = 42.8] [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da19350167630245085] 
\draw    (76,25) -- (76,75) ;
\draw [shift={(76,75)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(76,43.5)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(76,25)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da48014859020204725] 
\draw    (22,25) -- (76,25) ;
\draw [shift={(76,25)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(42.5,25)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(22,25)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da8489739329411121] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (76,25) -- (130,75) ;
\draw [shift={(130,75)}, rotate = 42.8] [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(98.23,45.58)}, rotate = 42.8] [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(76,25)}, rotate = 42.8] [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da017046498498133333] 
\draw    (130,25) -- (130,75) ;
\draw [shift={(130,75)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(130,43.5)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(130,25)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da5271051358345313] 
\draw    (76,25) -- (130,25) ;
\draw [shift={(130,25)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(96.5,25)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(76,25)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da5558516377031353] 
\draw    (22,75) -- (76,75) ;
\draw [shift={(76,75)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(42.5,75)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(22,75)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da8929723326353718] 
\draw    (76,75) -- (130,75) ;
\draw [shift={(130,75)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(96.5,75)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(76,75)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da21743094650805816] 
\draw    (76,75) -- (76,125) ;
\draw [shift={(76,125)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(76,93.5)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(76,75)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da6152345454151829] 
\draw    (22,25) -- (22,75) ;
\draw [shift={(22,75)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(22,43.5)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(22,25)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da6135522112818916] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (22,75) -- (76,125) ;
\draw [shift={(76,125)}, rotate = 42.8] [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(44.23,95.58)}, rotate = 42.8] [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(22,75)}, rotate = 42.8] [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;




\end{tikzpicture}     
        }
\end{figure}
By proposition \ref{prop:pos}, $\mathbb{F}P$ is isomorphic to $\mathbb{F}\tilde{P}$, where $\tilde{P}$ is the digraph below, where each square of $\tilde{P}$ is commutative:

\begin{figure}[bthp!]
\centering
        \resizebox{4cm}{!}{
  

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Straight Lines [id:da19350167630245085] 
\draw    (76,25) -- (76,75) ;
\draw [shift={(76,75)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(76,43.5)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(76,25)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da48014859020204725] 
\draw    (22,25) -- (76,25) ;
\draw [shift={(76,25)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(42.5,25)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(22,25)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da017046498498133333] 
\draw    (130,25) -- (130,75) ;
\draw [shift={(130,75)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(130,43.5)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(130,25)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da5271051358345313] 
\draw    (76,25) -- (130,25) ;
\draw [shift={(130,25)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(96.5,25)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(76,25)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da5558516377031353] 
\draw    (22,75) -- (76,75) ;
\draw [shift={(76,75)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(42.5,75)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(22,75)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da8929723326353718] 
\draw    (76,75) -- (130,75) ;
\draw [shift={(130,75)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(96.5,75)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(76,75)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da21743094650805816] 
\draw    (76,75) -- (76,125) ;
\draw [shift={(76,125)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(76,93.5)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(76,75)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da6152345454151829] 
\draw    (22,25) -- (22,75) ;
\draw [shift={(22,75)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(22,43.5)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(22,25)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;




\end{tikzpicture}         
        }
\end{figure}
\end{example}

\begin{theorem}[Fitting's lemma]\label{Fitting}
Let $R$ be a ring and $M\in\cat{Mod}_R$ with finite length. Then for any $\phi\in\End(M)$, there exists a positive integer $n$ such that $$M\cong\ker \phi^n\oplus \Ima \phi^n$$ 
\end{theorem}

\begin{figure}[bthp!]
\centering
        \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \resizebox{3cm}{!}{


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Straight Lines [id:da6593634943583064] 
\draw    (100,113) -- (100,47) ;
\draw [shift={(100,47)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(100,86.5)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da19483909403171662] 
\draw    (100,113) -- (163,113) ;
\draw [shift={(163,113)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(125,113)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(100,113)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da5399503195257365] 
\draw    (39,113) -- (100,113) ;
\draw [shift={(100,113)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(74.5,113)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(39,113)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da5048914562679376] 
\draw    (100,176) -- (100,113) ;
\draw [shift={(100,113)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(100,139.5)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(100,176)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;

% Text Node
\draw (165,92) node [anchor=north west][inner sep=0.75pt]   [align=left] {1};
% Text Node
\draw (108,34) node [anchor=north west][inner sep=0.75pt]   [align=left] {2};
% Text Node
\draw (41,91) node [anchor=north west][inner sep=0.75pt]   [align=left] {3};
% Text Node
\draw (107,168) node [anchor=north west][inner sep=0.75pt]   [align=left] {4};


\end{tikzpicture}
}
\caption{A poset has tame representation type.}%
\label{fig:2a}
         \end{subfigure}\hfill
        \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \resizebox{3cm}{!}{
        

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Straight Lines [id:da972900764614677] 
\draw    (100,113) -- (66,61.5) ;
\draw [shift={(66,61.5)}, rotate = 236.57] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(80.25,83.08)}, rotate = 56.57] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(100,113)}, rotate = 236.57] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da6593634943583064] 
\draw    (100,113) -- (127,55.5) ;
\draw [shift={(127,55.5)}, rotate = 295.15] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(115.63,79.72)}, rotate = 115.15] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da19483909403171662] 
\draw    (100,113) -- (163,113) ;
\draw [shift={(163,113)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(136.5,113)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(100,113)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da5399503195257365] 
\draw    (43,127.5) -- (100,113) ;
\draw [shift={(100,113)}, rotate = 345.73] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(65.2,121.85)}, rotate = 345.73] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(43,127.5)}, rotate = 345.73] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da5048914562679376] 
\draw    (72,175) -- (100,113) ;
\draw [shift={(100,113)}, rotate = 294.3] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(83.32,149.92)}, rotate = 294.3] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(72,175)}, rotate = 294.3] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da46171788233588984] 
\draw    (146,158.5) -- (100,113) ;
\draw [shift={(100,113)}, rotate = 224.69] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(127.62,140.32)}, rotate = 224.69] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(146,158.5)}, rotate = 224.69] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;

% Text Node
\draw (169,105) node [anchor=north west][inner sep=0.75pt]   [align=left] {1};
% Text Node
\draw (128,35) node [anchor=north west][inner sep=0.75pt]   [align=left] {2};
% Text Node
\draw (148,161.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {6};
% Text Node
\draw (54,42) node [anchor=north west][inner sep=0.75pt]   [align=left] {3};
% Text Node
\draw (28,122) node [anchor=north west][inner sep=0.75pt]   [align=left] {4};
% Text Node
\draw (61,178) node [anchor=north west][inner sep=0.75pt]   [align=left] {5};


\end{tikzpicture}
}
\caption{A poset has wild representation type.}
\label{fig:2b}
 \end{subfigure}\hfill
\caption{}
\end{figure}


==> mbboard.tex <==
% blackboard typefaces by Anthony Phan.
% file: mbboard.tex (\TeX' file for mbb's fonts)
% last modification: November 1st, 1999.
%
\catcode`@=11
%
% proofing?
%
\ifx\proofmode\undefined
	\def\symbol@message#1{\relax}%
	\def\symbol@mark#1#2{\relax}%
\else
	\def\symbol@message#1{\medbreak{\noindent\bf #1}
		\medskip\noindent\ignorespaces}%
	\def\symbolsp@cing#1{(\ifcase\number#1 ord\or op%
		\or bin\or rel\or open\or close\or punct%
		\or var\else ???\fi)}%
	\def\symbol@mark#1#2{$#1$ {\tt\string#1}
		\symbolsp@cing{#2},\ \ignorespaces}%
\fi
%
% Symbols declarations: \LaTeX-like commands
%
\def\hexnumber@#1{\ifcase\number#1 0\or 1\or 2\or 3\or 4%
	\or 5\or 6\or 7\or 8\or 9\or A\or B\or C\or D\or E\or F\fi}%
%
\def\DeclareMathSymbol#1#2#3#4{%
	\count255=#2\multiply\count255 by 16
	\advance\count255 by \csname#3fam\endcsname
	\multiply\count255 by 256\advance\count255 by #4
	\ifcat\noexpand#1\relax\mathchardef#1=\count255
	\else\expandafter
		\mathcode\expandafter`\csname#1\endcsname=\count255
	\fi\symbol@mark{#1}{#2}}
%
\def\gobble@quotes#1{\ifx#1"\else#1\fi}
%
\def\@DeclareMathDelimiter#1#2#3#4#5#6{%
	\edef#1{\noexpand\delimiter\noexpand"\gobble@quotes#2%
	\expandafter\hexnumber@\csname#3fam\endcsname\gobble@quotes#4%
	\expandafter\hexnumber@\csname#5fam\endcsname\gobble@quotes#6 }%
	\symbol@mark{#1}{#2}}
%
\def\@xDeclareMathDelimiter#1#2#3#4#5{%
	\count255=\csname#2fam\endcsname
	\multiply\count255 by 256\advance\count255 by #3
	\multiply\count255 by 16
	\advance\count255 by \csname#4fam\endcsname
	\multiply\count255 by 256\advance\count255 by #5
	\expandafter\delcode\expandafter`\csname#1\endcsname=\count255
	\symbol@mark{#1}{#2}}
%
\def\DeclareMathDelimiter#1{%
	\ifcat\noexpand#1\relax
	\def\Large@stuff{\noexpand\delimiter}%
	\expandafter\@DeclareMathDelimiter
	\else\expandafter\@xDeclareMathDelimiter\fi#1}
%
\def\DeclareMathRadical#1#2#3#4#5{%
	\edef#1{\noexpand\radical\noexpand"%
	\expandafter\hexnumber@\csname#2fam\endcsname\gobble@quotes#3%
	\expandafter\hexnumber@\csname#4fam\endcsname\gobble@quotes#5 }%
	\symbol@mark{#1.}{8}}
%
\def\DeclareMathAccent#1#2#3#4{%
        \edef#1{\noexpand\mathaccent\noexpand"%
	\expandafter\hexnumber@\csname#3fam\endcsname\gobble@quotes#4 }%
	\symbol@mark{#1.}{8}}
%
% loading blackboard fonts
%
\font\twelvembb=mbb12 \font\tenmbb=mbb10
\font\ninembb=mbb9    \font\eightmbb=mbb8
\font\sevenmbb=mbb7   \font\sixmbb=mbb6
\font\fivembb=mbb5
%
\skewchar\tenmbb="7F   \skewchar\ninembb="7F \skewchar\eightmbb="7F 
\skewchar\sevenmbb="7F \skewchar\sixmbb="7F  \skewchar\fivembb="7F 
\hyphenchar\tenmbb="2D   \hyphenchar\ninembb="2D \hyphenchar\eightmbb="2D 
\hyphenchar\sevenmbb="2D \hyphenchar\sixmbb="2D  \hyphenchar\fivembb="2D 
%
\newfam\mbbfam
%
% Initialization
% (make changes in your own file if you want different sizes)
%
\textfont\mbbfam=\tenmbb  \scriptfont\mbbfam=\sevenmbb
\scriptscriptfont\mbbfam=\fivembb  \def\mbb{\fam\mbbfam\tenmbb}
\def\mathbb#1{{\fam\mbbfam#1}}
%
\input mbboard.dcl
%
\catcode`@=12
\let\proofmode=\undefined
\endinput




